DAE-Former: Dual Attention-guided Efficient Transformer for Medical Image Segmentation

Transformers have recently gained attention in the computer vision domain due to their ability to model long-range dependencies. However, the self-attention mechanism, which is the core part of the Transformer model, usually suffers from quadratic computational complexity with respect to the number of tokens. Many architectures attempt to reduce model complexity by limiting the self-attention mechanism to local regions or by redesigning the tokenization process. In this paper, we propose DAE-Former, a novel method that seeks to provide an alternative perspective by efficiently designing the self-attention mechanism. More specifically, we reformulate the self-attention mechanism to capture both spatial and channel relations across the whole feature dimension while staying computationally efficient. Furthermore, we redesign the skip connection path by including the cross-attention module to ensure the feature reusability and enhance the localization power. Our method outperforms state-of-the-art methods on multi-organ cardiac and skin lesion segmentation datasets without requiring pre-training weights. The code is publicly available at https://github.com/mindflow-institue/DAEFormer.

==> commented_passages.tex <==
% \begin{abstract}
% The transformer architecture has gained traction in the computer vision domain and is challenging CNNs because of its ability to model long-range dependencies.
% Many architectures attempt to reduce model complexity by limiting the self-attention mechanism to local regions or by applying shifted windows.
% We propose the \transformerlong, a U-Net-like hierarchical pure transformer architecture that models spatial and channel relations across the whole feature dimension while staying computationally efficient.
% Efficient attention allows us to compute spatial self-attention across the whole input feature because it has linear complexity. We combine it with transpose attention in a dual attention block
% to gain a powerful representation across all input dimensions. We also introduce skip connection cross attention to smartly fuse features from different layers in our U-Net-like architecture. Our
% architecture achieves state-of-the-art performance on the Synapse segmentation dataset and the Skin Lesion dataset. The code is available at \githublink.
    
% passage 1    
Deep learning networks perform exceedingly well in medical imaging, surpassing non-deep state-of-the-art methods.
However, an immense volume of data is required to train and achieve good generalization with the large amount of network parameters. Another issue is that large (annotated) datasets for medical image segmentation are not readily available. Unfortunately, per pixel labeling is necessary for medical image segmentation, making annotation even more tedious. Fully convolutional neural network (FCN) was one of the pioneer networks utilized for image segmentation.
The U-Net by Ronneberger et al. enhances the FCN architecture. Unlike FCN, U-Net performs well on segmentation tasks without the need for huge training sets. The U-Net is made up of an encoder and decoder branch. The encoder produces several feature maps with reduced dimensionality. The decoder employs up-convolutions to generate segmentation maps (with the same size as the input). Many improvements of the U-Net architecture exist. Some of them use another processing step (e.g. attention gates) on the feature maps in the skip connection before concatenation. The main flaw of these architectures is that the processing step is applied separately to each of the two feature maps. The features are only concatenated. Instead, a processing step using feature fusion to find the most salient components of both feature maps could improve the output representation.

% passage 2:
Several Expansions to the U-Net have been proposed to enhance the performance of the network~\cite{zahangir2018recurrent,asadi2020multi,azad2019bi,fan2020pranet,feyjie2020semi,schlemper2019attention,zhou2018unet++}.
These methods inject attention mechanisms, recurrent residual strategies, or other non-linear functions into the convolutional layers of U-Net in order to augment the original architecture.
All of them extract features based on texture, whereas extracting features based on shape is also beneficial. Low-frequency information is carried by shape information, which the abovementioned methods fail to utilize. It is proven that exploiting shape information in CNNs by fine-tuning the input images can boost the representational power of the network~\cite{geirhos2018imagenet}. In spite of that, it is still a challenging task to construct a CNN that reduces the impact of high-frequency parts while profitting from low-frequency information.
The squeeze and excitation module~\cite{SEnet} shows that this problem can be solved by recalibrating frequency representations through a channel-wise attention mechanism. We propose a weighted combination function that accumulates the features of all levels of X, weighing each level based on the impact on the final result. Thus, the network learns to pinpoint informative and relevant features and eliminates redundant and noisy ones by using global embedding information of the channels.




% % Medical imaging important, especially segmentation
% Medical image segmentation has become one of the major challenges in computer vision. In order for physicians to accurately monitor diseases, visualize injuries and select the correct treatment,
% stable and precise image segmentation algorithms are highly necessary \cite{antonelli2022medical}. Telesurgery and robotic surgery heavily depend on segmentation as well \cite{hagn2010dlr}.
% % CNNs de-facto standard

% CNNs have become the de facto standard for medical image segmentation. ResNet~\cite{resnet} and U-Net~\cite{ronneberger2015unet} are two prevalent CNN architectures for segmentation.
% The U-Net architecture is popular due to its symmetry, multiscale representation, and the ability to localize semantic features more easily through skip connections. CNNs have one major drawback, however.
% By design, CNNs have a limited receptive field due to the locality of the convolution operation. The global context and long range dependencies are not captured.
% Attention and Transformers
To counteract the drawbacks of CNNs, the attention mechanism was introduced.~\cite{oktay2018attention,SEnet,woo2018cbam,xu2015show} are a few of the examples that show how the attention mechanism can improve existing architectures.
Attention also opened the opportunity for the transformer architecture~\cite{vaswani2017attention}. Due to its success in machine translation, the architecture was ported to computer vision as the Vision Transformer (ViT)~\cite{dosovitskiy2020vit}.



Another issue is that large (annotated) datasets for medical image segmentation are not readily available.



% We aim at efficiently computing both spatial and channel attention. Unlike previous methods, which restrict the self-attention mechanism in some way to deal with the quadratic overhead,
% we utilize efficient attention and transpose attention, both of which have linear complexity with regards to the number of tokens.
% We combine transpose and efficient attention in a dual attention module to first recalibrate the feature dimension and then compute global context.
% Skip connection cross attention fuses features from different layers by computing the context between encoder and decoder features.
% First, we present the overall architecture. We then show the two components of the dual attention module. Thirdly, we explain efficient dual attention. Lastly, skip connection cross attention is introduced.

% passage 3:
The encoder feature maps have a higher resolution than the feature maps from the patch merging layer, which in turn encompass more semantic information. Usually, skip connection features are concatenated. Instead, we predict that fusing these two different feature maps using nonlinear functions will produce more precise segmentation maps in the output. To this end, we expand the U-Net architecture by implementing SCCA in the skip connection to combine the two types of feature maps.



% Ding et al.~\cite{ding2022davit} show that spatial and channel attention combined as dual attention can capture more context than spatial attention alone. We therefore construct a dual transformer block that combines
% transpose (channel) attention and efficient (spatial) attention. The structure of the efficient dual attention block is shown in~\figureref{fig:proposed_method} (b).

% Each image's ground truth segmentation map includes 8 classes: \textit{Aorta, Gallbladder, Kidney(L), Kidney(R), Liver, Pancreas, Spleen, Stomach}.
% The dataset is preprocessed~\cite{chen2021transunet} and each image is size $224 \times 224$.
% For evaluation, we use the Dice Similarity Coefficient(DSC) as well as the average Hausdorff Distance (HD). The training was performed on a high performance computing cluster using Python 3.10.4, Pytorch 1.12.1 and Cuda toolkit 11.6.



\begin{align}
    L_{dice}(y, \hat{p}) & = 1 - \frac{2y\hat{p} + 1}{y + \hat{p} +1}      \\
    L_{ce}(y, \hat{y})   & =  - (y log(\hat{y}) + (1 - y)log(1 - \hat{y})) \\
    L_{total}            & = 0.6 \cdot L_{dice} + 0.4 \cdot L_{ce}
\end{align}


$n$ is the input size, $d$ the embedding dimension, $d_{k}$ and $d_{v}$ are the embedding dimension of the keys and values.

% passage skin
\subsubsection{Quantitative Results}
The results on the ISIC and PH$^{2}$ datasets are presented in~\tableref{tab:quantitative}. In order to show the effectiveness of our approach, we compare it with the results of concurrent work. Our method surpasses others in terms of DSC for all three datasets. 

\subsubsection{Qualitative Results}
Visualizations of the segmentation masks for all three datasets are shown in~\figref{fig:skin_visualization}. We observe that our model finds large coherent areas well.


The efficiency with regards to the number of parameters is mentioned in~\tableref{tab:parameters_synapse} and will be discussed further below.


\section{Model Configuration}
All models were trained with the following configuration: The model consists of 3 encoder and decoder layers each. 2 consecutive dual transformer blocks are preceded by a
patch merging block in each encoder layer, and followed by a patch expanding block in each decoder layer. The three decoder layers excluding the lowest also contain an SCCA module after the patch expanding, which has both the
decoder and skip connection features as input. The SCCA module is followed by an extra linear layer to project the embedding dimension back to the block input dimension (the output of the SCCA block is double the input dimension). All attention modules are single head.



\section{Ablation Studies}

In this section, different ablation studies regarding the structure of dual attention are presented.

\subsection{Dual Attention}


% \subsection{Effects of Model Depth and Model Scaling}

% To explore the effects of model depth and model scaling, the model was trained with different depths and blocks per layer, as shown in \tableref{tab-model-scaling}. The dataset used was the Synapse dataset,
% with $224 \times 224$ as the image size. Because of the small image size, increasing the amount of layers does not work as the lowest patch size for four layers is already seven, which cannot be further reduced.
% \begin{table}[!h]
%     \centering
%     \begin{tabular}{ c c c c c}
%         \toprule
%         \textbf{\# of Layers} & \textbf{\# of Blocks per Layer} & \textbf{Params}  & \textbf{DSC} & \textbf{HD}    \\
%         \hline
%         3        & 2                  & 48.1 M  & 82.66           & 26.79 \\
%         4        & 2                  & 48.5 M  & 81.51           & 17.62 \\
%         4        & 3                  & 67.3 M  & 80.77           & 23.51 \\
%         4        & 4                  & 86.1 M  & 82.82           & 20.43 \\
%         4        & 5                  & 104.9 M & 80.11           & 34.60 \\
%         4        & 6                  & 123.7 M & 80.55           & 28.17 \\
%         4        & 7                  & 142.4 M & 82.31           & 21.68 \\
%         4        & 8                  & 161.2 M & 81.25           & 25.79 \\
%         \hline
%     \end{tabular}
%     \caption{Performance comparison for different model depths.}\label{tab-model-scaling}
% \end{table}
% Intuitively, one might assume that the performance increases monotonically as the model size increases. This is not the case, instead the performance stagnates. This is most likely due to the attention maps being too similar in deeper layers.
% The model does not learn any new information and the performance cannot increase with higher model depth.


